Accurate Power Spectrum Estimation toward Nyquist limit

The power spectrum, as a statistic in Fourier space, is commonly numerically calculated using the fast Fourier transform method to efficiently reduce the computational costs. To alleviate the systematic bias known as aliasing due to the insufficient sampling, the interlacing technique was proposed. We derive the analytical form of the shot noise under the interlacing technique, which enables the exact separation of the Poisson shot noise from the signal in this case. Thanks to the accurate shot noise subtraction, we demonstrate an enhancement in the accuracy of power spectrum estimation, and compare with the other widely used estimators in community. The good performance of our estimation allows an abatement in the computational cost by using low resolution and low order mass assignment scheme in the analysis for huge surveys and mocks.

==> halo_full_sample.tex <==

\begin{figure*}[htbp]
\centerline{\includegraphics[width=\fsize]{fig3/halo002_compare_cic_100percent_inorder.png}
\includegraphics[width=\fsize]{fig3/halo002_compare_tsc_100percent_inorder.png}}
\caption{The power spectrum of the full halo sample. The symbols have the same meaning as those in Figure~\ref{fig:full_dm}.}
\label{fig:100pc}

\end{figure*}

\sout{Based on the aforementioned samples, we test the results using the CIC and TSC window functions with a grid size of $N_g = 200$. }
\sout{The mesh size is $3\,\mpch$ and the corresponding Nyquist frequency $k_N=1.047\,\hmpc$.}
\sout{We choose this relatively large mesh size under the consideration that for Stage-IV surveys a cubic box covering the whole footprint may reach $(6\,\gpch)^3$ and the analysis in performed on $2000^3$ mesh.}
\sout{We compare the differences among the four estimators mentioned above.}
\sout{To reflect the magnitude of systematic biases for the samples, we treat the results from a 10 times higher sampling rate, $N_g = 2000$, as the true values for the power spectrum. }
\sout{We have confirmed that, at this high sampling frequency, the power spectrum results from different estimators with different window functions are overlapping with each other below the Nyquist frequency of $N_g=200$ mesh.}
\sout{Therefore, we can consider it as the true value for a low sampling frequency result.}
For the full sample with a total count of $N_s = 2,413,300$ and a number density of $n_s = 1.12\times 10^{-2}\,\hmpct$ , the power spectrum results are shown in Figure \ref{fig:100pc}.
\brown{The power spectrum is lower on large scales compared to the dark matter sample of the same size, while the estimator's error remains generally consistent.}
Under the CIC window, Eq.\,(\ref{eqn:noint-shot-win}) yields an overestimated result, with an error exceeding 10\% at $k = k_N$. Eq.\,(\ref{eqn:noint-win-shot}) gives an underestimated result, with an error of around 10\% near $k = k_N$. Both errors far exceed the level of statistical fluctuations. However, with the interlacing technique, Eq.\,(\ref{eqn:int-win-shot}) exhibits errors larger than statistical fluctuations only at the scale of $k = 0.9k_N$, reaching around 1\% at $k = k_N$. Meanwhile, Eq.\,(\ref{eqn:int-shot-win}) maintains an error within 0.1\%.

Under the TSC window, the errors are reduced. Eq.\,(\ref{eqn:noint-shot-win}) provides an overestimated result, with an error of approximately 10\% at $k = k_N$. Eq.\,(\ref{eqn:noint-win-shot}) yields an underestimated result, with an error of around 5\% near $k = k_N$. Both errors still significantly exceed the level of statistical fluctuations. However, with the interlacing technique, both Eq.\,(\ref{eqn:int-shot-win}) and Eq.\,(\ref{eqn:int-win-shot}) exhibit errors smaller than the level of statistical fluctuations within the Nyquist frequency. Specifically, Eq.\,(\ref{eqn:int-shot-win}) has an error within 0.002\% at $k = k_N$, while Eq.\,(\ref{eqn:int-win-shot}) has an error within 0.1\%.
\sout{
We can observe that adopting higher-order window functions with the interlacing technique effectively reduces estimation errors,
which is the main conclusion of \cite{Sefusatti16}.
However, when not using the interlacing technique, the reduction of errors with higher-order window functions is not significant. In terms of performance under the interlacing technique, Eq.\,(\ref{eqn:int-shot-win}) performs better than Eq.\,(\ref{eqn:int-win-shot}).}


==> halo_random_10percent.tex <==
\begin{figure*}[htbp]
\includegraphics[width=\fsize]{fig3/halo002_compare_cic_10percent_random.png}
\includegraphics[width=\fsize]{fig3/halo002_compare_tsc_10percent_random.png}
\caption{The power spectrum of the 10\% randomly sampled data. The symbols have the same meaning as those in Figure~\ref{fig:full_dm}.}
\label{fig:10percent_random}
\end{figure*}

We perform the same calculations as in Section~\ref{sec:fulsample}, but this time we randomly select\sout{ed} 10\% of the samples from the entire sample, resulting in a sample size of $N_s = 241,330$. The sample number density is $n_s = 1.12\times 10^{-3} \text{ Mpc}^{-3} h^3$. We obtain the power spectrum with the same amplitude as in Section~\ref{sec:fulsample}, 
but the corresponding shot noise term $\frac{1}{N}$ is ten times larger after down-sampling,
resulting in larger fluctuations on top of the original power spectrum. The results are shown in Figure \ref{fig:10percent_random}.

Under the CIC window, Eq.\,(\ref{eqn:noint-shot-win}) provides an overestimated result, and Eq.\,(\ref{eqn:noint-win-shot}) yields an underestimated result. Both errors exceed 10\% near $k = k_N$, far exceeding the level of statistical fluctuations. With the interlacing technique, Eq.\,(\ref{eqn:int-win-shot}) exhibits errors exceeding the level of statistical fluctuations below the scale of $k = 0.7k_N$, reaching 10\% at $k = k_N$, while Eq.\,(\ref{eqn:int-shot-win}) maintains an error within 1\% despite larger fluctuations.

Under the TSC window, the errors are improved. Eq.\,(\ref{eqn:noint-shot-win}) provides an overestimated result, with an error of approximately 10\% at $k = k_N$. Eq.\,(\ref{eqn:noint-win-shot}) yields an underestimated result, with an error of around 5\% near $k = k_N$. Both errors still significantly exceed the level of statistical fluctuations. With the interlacing technique, Eq.\,(\ref{eqn:int-shot-win}) exhibits errors smaller than statistical fluctuations within the Nyquist frequency. Specifically, it has an error below 0.2\% at $k = k_N$, while Eq.\,(\ref{eqn:int-win-shot}) exceeds the level of statistical fluctuations and reaches 0.7\%.
\sout{
Compared to the result in Section~\ref{sec:fulsample}, the systematic bias is significantly larger due to the lower sample density, especially for the estimators with inexact shot noise subtraction.
We can see that under the interlacing technique, the estimation Eq.\,(\ref{eqn:int-shot-win}) still performs better than Eq.\,(\ref{eqn:int-win-shot}).}


%\begin{figure*}[htbp]
%\includegraphics[width=\fsize]{fig3/halo002_compare_cic_10percent_random_2Nyquist.png}
%\caption{Same as the left panel of the Figure~\ref{fig:10percent_random}, but with a larger range of the bottom panel, merely for showcasing. }
%\label{fig:showcase}
%\end{figure*}

==> halo_random_1percent.tex <==

\begin{figure*}[htbp]
\centerline{\includegraphics[width=\fsize]{fig3/halo002_compare_cic_1percent_random.png}
\includegraphics[width=\fsize]{fig3/halo002_compare_tsc_1percent_random.png}}
\caption{The power spectrum of the 1\% randomly sampled data. The symbols have the same meaning as those in Figure~\ref{fig:full_dm}.}
\label{fig:1percent_random}
\end{figure*}

We randomly select a sparse sample from the total dataset, consisting of 1\% of the total sample size, which corresponds to $N_s=24, 133$ halos. The number density of this sparse sample is $n_s=1.12\times 10^{-4} \,\text{Mpc}^{-3} h^3$. We perform the same computation as described in Section~\ref{sec:fulsample} on this sparse sample, and we expect to obtain power spectra with the same amplitude as in Section~\ref{sec:fulsample}. However, due to the sparsity of this sample, the resulting power spectrum will exhibit even larger fluctuations compared to the results in Section~\ref{sec:10pcrandom}. 
The results are presented in Figure~\ref{fig:1percent_random}.
Under the CIC window, Eq.\,(\ref{eqn:noint-win-shot}) overestimates the results, while Eq.\,(\ref{eqn:noint-shot-win}) underestimates them. Both estimations show errors of around 10\% near $k=0.7k_N$, which greatly exceeds the size of statistical fluctuations.
Under the interlacing technique, Eq.\,(\ref{eqn:int-win-shot}) exhibits errors of over 50\% at $k=0.9k_N$, while Eq.\,(\ref{eqn:int-shot-win}) exhibits errors of over 50\% near the Nyquist frequency.
Under the TSC window, Eq.\,(\ref{eqn:noint-win-shot}) overestimates the results, with an error of over 50\% at $k=0.95k_N$, and Eq.\,(\ref{eqn:noint-shot-win}) underestimates them, with an error within 50\% near the Nyquist frequency. Both estimations still greatly exceed the size of statistical fluctuations.
Although under the interlacing technique the errors still exceed the size of statistical fluctuations. Eq.\,(\ref{eqn:int-shot-win}) exhibits errors within 5\% near the Nyquist frequency, while Eq.\,(\ref{eqn:int-win-shot}) exhibits errors of around 15\% near the same frequency. It can be seen that under this sampling scheme, the estimation using Eq.\,(\ref{eqn:int-shot-win}) still demonstrates a precision advantage.

